Variant tolerant read mapping using min-hashing

DNA read mapping is a ubiquitous task in bioinformatics, and many tools have been developed to solve the read mapping problem. However, there are two trends that are changing the landscape of readmapping: First, new sequencing technologies provide very long reads with high error rates (up to 15%). Second, many genetic variants in the population are known, so the reference genome is not considered as a single string over ACGT, but as a complex object containing these variants. Most existing read mappers do not handle these new circumstances appropriately. We introduce a new read mapper prototype called VATRAM that considers variants. It is based on Min-Hashing of q-gram sets of reference genome windows. Min-Hashing is one form of locality sensitive hashing. The variants are directly inserted into VATRAMs index which leads to a fast mapping process. Our results show that VATRAM achieves better precision and recall than state-of-the-art read mappers like BWA under certain cirumstances. VATRAM is open source and can be accessed at https://bitbucket.org/Quedenfeld/vatram-src/.

==> exp_real_se.tex <==
\begin{figure}[p]
\pgfplotsset{footnotesize,width=13cm,height=4.6cm}
%\pgfplotsset{footnotesize,samples=10}
\begin{center}
\setlength{\tabcolsep}{0mm}
\begin{tabular}{r}
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0,ymax=1,
%ymin=.92,
enlarge x limits=0.2,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
ylabel style={align=center},
ylabel=Korrekt gemappt,
yticklabel=
	\pgfmathparse{100*\tick}
	\pgfmathprintnumber{\pgfmathresult}\,\%,
yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
xtick=data,
scaled ticks=false,
legend columns=4,
legend entries={BWA-MEM, BWA-MEM (Edit-Distanz), BWA-SW, Bowtie2, VATRAM, VATRAM (ohne Varianten), mrsFast-Ultra},
legend cell align=left,
%legend pos=south east,
legend to name=leg:exp:comp:const:rm:balken
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_corr.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_corr.dat};
\end{axis}
\end{tikzpicture}
\\
\pgfplotsset{width=9.8cm}
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0.88,ymax=1,
%ymin=.92,
enlarge x limits=0.3,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
ylabel style={align=center},
ylabel={Korrekt gemappt\\ (Details)},
yticklabel=
	\pgfmathparse{100*\tick}
	\pgfmathprintnumber{\pgfmathresult}\,\%,
yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
xtick=data,
scaled ticks=false,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_corr_abc.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_corr_abc.dat};
\end{axis}
\end{tikzpicture}
%
\pgfplotsset{width=4.4cm}
\begin{tikzpicture}
\begin{axis}[
ybar,
ymin=0.48,ymax=.6,
%ymin=.92,
enlarge x limits=0.21,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
%ylabel=Korrekt gemappt,
yticklabel=
	\pgfmathparse{100*\tick}
	\pgfmathprintnumber{\pgfmathresult}\,\%,
yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
xtick=data,
scaled ticks=false,
ylabel near ticks, yticklabel pos=right,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_corr_d.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_corr_d.dat};
\end{axis}
\end{tikzpicture}
\hspace{-1cm}
\\
\pgfplotsset{width=13cm}
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0,
%ymin=.92,
enlarge x limits=0.2,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
ylabel=Falsch gemappt,
yticklabel=
	\pgfmathparse{100*\tick}
	\pgfmathprintnumber{\pgfmathresult}\,\%,
yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
xtick=data,
scaled ticks=false,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_wrong.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_wrong.dat};
\end{axis}
\end{tikzpicture}
\\
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0,
%ymin=.92,
enlarge x limits=0.2,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
ylabel=Laufzeit,
%yticklabel=
%	\pgfmathparse{100*\tick}
%	\pgfmathprintnumber{\pgfmathresult}\,\%,
%yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
%yticklabels={,,},
xtick=data,
scaled ticks=false,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_tbase.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_tbase.dat};
\end{axis}
\end{tikzpicture}
\\
\pgfplotsset{width=9.8cm}
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0,ymax=0.4,
%ymin=.92,
enlarge x limits=0.3,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
ylabel=Laufzeit (Details),
%yticklabel=
%	\pgfmathparse{100*\tick}
%	\pgfmathprintnumber{\pgfmathresult}\,\%,
%yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
%yticklabels={,,},
xtick=data,
scaled ticks=false,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_tbase_abc.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_tbase_abc.dat};
\end{axis}
\end{tikzpicture}
%
\pgfplotsset{width=4.4cm}
\begin{tikzpicture}%[trim axis left]
\begin{axis}[
ybar,
ymin=0,%ymax=0.5,
%ymin=.92,
enlarge x limits=0.21,
bar width=0.25cm,
%xlabel=$q$-Gramm-Hashfunktion,
%ylabel=Laufzeit (Details),
%yticklabel=
%	\pgfmathparse{100*\tick}
%	\pgfmathprintnumber{\pgfmathresult}\,\%,
%yticklabel style={/pgf/number format/.cd,fixed,precision=2},
%title={Variation der $q$-Gramm-Länge},
symbolic x coords={ERR385811, ERR281333, SRR1374471, ERR967952},
%x tick label style={rotate=90,anchor=east},
%yticklabels={,,},
xtick=data,
scaled ticks=false,
ylabel near ticks, yticklabel pos=right,
]
\addplot[barstyleBWA]
 table[x=set,y=bwa] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleBWAedit]
 table[x=set,y=bwaedit] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleBWAsw]
 table[x=set,y=bwasw] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleBowtie]
 table[x=set,y=bowtie2] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleVATRAM]
 table[x=set,y=vatram] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleVATRAMnovar]
 table[x=set,y=vatramnovar] {data/exp_comp_const_real_tbase_d.dat};
\addplot[barstyleMRSfast]
 table[x=set,y=mrsfast] {data/exp_comp_const_real_tbase_d.dat};
\end{axis}
\end{tikzpicture}
\hspace{-.5cm}
\end{tabular}
\ref*{leg:exp:comp:const:rm:balken}
\end{center}
\caption{Real single-end reads with constant length. More information about the data sets can be found in table~\ref{tab:exp:comp:realdata}. The last dritte Datensatz (SRR1374471) führte beim Readmapper \emph{mrsFAST-Ultra} aus ungeklärter Ursache zu einem Absturz.}
\label{fig:exp:real:se}
\end{figure}
